Diffusion-Based Neural Network Weights Generation

Transfer learning has gained significant attention in recent deep learning research due to its ability to accelerate convergence and enhance performance on new tasks. However, its success is often contingent on the similarity between source and target data, and training on numerous datasets can be costly, leading to blind selection of pretrained models with limited insight into their effectiveness. To address these challenges, we introduce D2NWG, a diffusion-based neural network weights generation technique that efficiently produces high-performing weights for transfer learning, conditioned on the target dataset. Our method extends generative hyper-representation learning to recast the latent diffusion paradigm for neural network weights generation, learning the weight distributions of models pretrained on various datasets. This allows for automatic generation of weights that generalize well across both seen and unseen tasks, outperforming state-of-the-art meta-learning methods and pretrained models. Moreover, our approach is scalable to large architectures such as large language models (LLMs), overcoming the limitations of current parameter generation techniques that rely on task-specific model collections or access to original training data. By modeling the parameter distribution of LLMs, D2NWG enables task-specific parameter generation without requiring additional fine-tuning or large collections of model variants. Extensive experiments show that our method consistently enhances the performance of diverse base models, regardless of their size or complexity, positioning it as a robust solution for scalable transfer learning.

==> figures/introductionfigure.tex <==
\begin{figure}[t!]
\centering
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/recognizance1_plots_new.pdf}
        \caption{\textbf{Dessert Dataset}} %Best initialization for no fine-tuning}
        \label{intro:a}
    \end{subfigure} 
    \begin{subfigure}{0.23\textwidth}
	\centering
	\includegraphics[width=\linewidth]{images/gemstones-images_lsind18_plots_new.pdf}
	\captionsetup{justification=centering,margin=0.5cm}
	\caption{\textbf{Gemstones Dataset}}%Best initialization for fine-tuning}
 \label{intro:b}
    \end{subfigure}
    \caption{\small We train D2NWG on a modelzoo generated from the training split of the Kaggle Dataset of ~\citep{Jeong2021TaskAdaptiveNN} and generate weights directly for the datasets in the test split. In Figure~\ref{intro:a} we sample the full set of weights using D2NWG (without any finetuning) conditioned on the dataset encoding of the Dessert dataset. For the baselines, we finetune them on the full Dessert dataset. In Figure~\ref{intro:b}, we again perform dataset-conditioned sampling with D2NWG and fintune it, together with a model pretrained on ImageNet and a randomly initialized model (RandInit) for 50 epochs. As can be seen, D2NWG can sample high performing weights for unseen datasets and achieves better convergence rate when the sampled weights are finetuned. The full set of results for Kaggle dataset is provided in Table~\ref{tab2} in the experimental section.}
    \label{fig:intro}
    \vspace{-0.15in}
\end{figure}

==> figures/kaggle.tex <==
\begin{figure*}[t!]
\centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/group_0.pdf}
        \caption{Group 1}
    \end{subfigure} 
    \begin{subfigure}{0.24\textwidth}
	\centering
	\includegraphics[width=\linewidth]{images/group_1.pdf}
	\captionsetup{justification=centering,margin=0.5cm}
	\caption{Group 2}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
	\centering
	\includegraphics[width=\linewidth]{images/group_2.pdf}
	\captionsetup{justification=centering,margin=0.5cm}
	\caption{Group 3}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
	\centering
	\includegraphics[width=\linewidth]{images/group_3.pdf}
	\captionsetup{justification=centering,margin=0.5cm}
	\caption{Group 4}
    \end{subfigure}
    \caption{\small Average accuracy evolution of fine-tuning for 50 epochs with sampled weights. group 1: Gemstones(gem), Dog Breeds(ucf), Japanese Characters(kuz). group 2: Colorectal Histology(col), Drawing(ml2), group 3: Dessert(rec), Alien vs Predator(ali), honey-bee-pollen(hon), group 4: COVID-19(cov), Speed Limit Signs(drr). The corresponding plots are named using the first 3 letter of each dataset instead of using the full name description.}
   
    \label{fig:kagapp}
\end{figure*}

==> tables/convergence_speed.tex <==
% \begin{table}[t]
%\begin{wraptable}{r}{0.5\columnwidth}
%\vspace{-0.15in}
%\caption{
%\textbf{Convergence Speed Comparison} Sampled weights from S\textsubscript{\texttt{KDE30}}~\citep{schurholtHyperRepresentationsGenerativeModels2022} and our method are evaluated on the test set after 0 (meaning no optimization steps), 1 and 25 epochs of training on the training set. The Pretrained baseline is trained on the training set for a total of 50 epochs.}
%% \vspace{-0.2in}
%
%\begin{center}
%
%\resizebox{0.5\columnwidth}{!}{
%\begin{tabular}{lccccc}
%\toprule
%Model &Epoch &  MNIST & SVHN & CIFAR-10 & STL-10 \\
%\hline
%Pretrained models& 25 & \textbf{82.82$\pm$ 1.38}& \textbf{67.57$\pm$ 0.59}& \textbf{44.68$\pm$ 3.15} & \textbf{35.99$\pm$ 1.15}\\
%S\textsubscript{\texttt{KDE30}} & 0& 69.73$\pm$ 5.12& 50.25$\pm$ 6.12 & 26.06$\pm$ 3.01& 17.20$\pm$ 3.43\\
%D2NWG (Ours)   & 0& 78.10$\pm$0.29& 58.92$\pm$ 0.76& 38.23$\pm$ 5.45& 22.74$\pm$ 2.08\\
%\hline
%Pretrained models& 26& \textbf{85.50$\pm$ 0.99}& 67.79$\pm$ 1.05& 44.81$\pm$ 3.20& \textbf{36.28$\pm$ 1.18}\\
%S\textsubscript{\texttt{KDE30}} & 1& 82.69$\pm$ 0.81& 70.45$\pm$ 0.92& 44.75$\pm$ 0.81& 28.42$\pm$ 1.53\\
%D2NWG (Ours)  & 1& 83.25$\pm$ 0.25& \textbf{73.11$\pm$0.24} & \textbf{46.88$\pm$ 0.85}& 34.39$\pm$ 0.51\\
%\hline
%Pretrained models& 50& 95.70$\pm$ 0.36& 74.49$\pm$ 1.53& 49.25$\pm$ 3.00& 39.39$\pm$0.89\\
%S\textsubscript{\texttt{KDE30}} & 25& 95.70$\pm$ 0.30& 74.69$\pm$ 0.70 & 49.14$\pm$ 0.65 & 39.14$\pm$ 0.76\\
%D2NWG (Ours)   & 25& \textbf{96.17$\pm$0.0.33} & \textbf{74.75}$\pm$ 0.33&\textbf{ 49.48$\pm$ 0.97}& \textbf{39.43$\pm$ 0.13}\\
%\bottomrule
%\end{tabular}
%}
%\end{center}
%\label{table2}
%\vspace{-0.2in}
%% \end{table}
%\end{wraptable}

\begin{table*}[t]
\caption{\textbf{Convergence Speed Comparison} Sampled weights from S\textsubscript{\texttt{KDE30}}~\citep{schurholtHyperRepresentationsGenerativeModels2022} and our method are evaluated on the test set after 0 (meaning no optimization steps), 1 and 25 epochs of training on the training set. The Pretrained baseline is trained on the training set for a total of 50 epochs.}

\begin{center}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
Model &Epoch &  MNIST & SVHN & CIFAR-10 & STL-10 \\
\hline
Pretrained models& 25 & \textbf{82.82$\pm$ 1.38}& \textbf{67.57$\pm$ 0.59}& \textbf{44.68$\pm$ 3.15} & \textbf{35.99$\pm$ 1.15}\\
S\textsubscript{\texttt{KDE30}} & 0& 69.73$\pm$ 5.12& 50.25$\pm$ 6.12 & 26.06$\pm$ 3.01& 17.20$\pm$ 3.43\\
D2NWG (Ours)   & 0& 78.10$\pm$0.29& 58.92$\pm$ 0.76& 38.23$\pm$ 5.45& 22.74$\pm$ 2.08\\
\hline
Pretrained models& 26& \textbf{85.50$\pm$ 0.99}& 67.79$\pm$ 1.05& 44.81$\pm$ 3.20& \textbf{36.28$\pm$ 1.18}\\
S\textsubscript{\texttt{KDE30}} & 1& 82.69$\pm$ 0.81& 70.45$\pm$ 0.92& 44.75$\pm$ 0.81& 28.42$\pm$ 1.53\\
D2NWG (Ours)  & 1& 83.25$\pm$ 0.25& \textbf{73.11$\pm$0.24} & \textbf{46.88$\pm$ 0.85}& 34.39$\pm$ 0.51\\
\hline
Pretrained models& 50& 95.70$\pm$ 0.36& 74.49$\pm$ 1.53& 49.25$\pm$ 3.00& 39.39$\pm$0.89\\
S\textsubscript{\texttt{KDE30}} & 25& 95.70$\pm$ 0.30& 74.69$\pm$ 0.70 & 49.14$\pm$ 0.65 & 39.14$\pm$ 0.76\\
D2NWG (Ours)   & 25& \textbf{96.17$\pm$0.0.33} & \textbf{74.75}$\pm$ 0.33&\textbf{ 49.48$\pm$ 0.97}& \textbf{39.43$\pm$ 0.13}\\
\bottomrule
\end{tabular}			
\end{center}
\label{table2}
\end{table*}


==> tables/cross_arch.tex <==


\begin{table}[h]
\centering
\begin{tabular}{lllll}
\toprule
\textbf{Method}  & \textbf{ResNet20 (Unseen)} & \textbf{ResNet32 (Seen)} & \textbf{ResNet44 (Unseen)} & \textbf{ResNet56 (Unseen)} \\ 
\midrule
\textbf{Pretrained} & 92.60 & 93.53 & 94.01 & 94.37 \\ 
\midrule
\textbf{RandInit}   & 10.00 & 10.00 & 10.00 & 10.00 \\
\midrule
\textbf{Ours}       & 53.62 & 93.48 & 86.52 & 83.39 \\ 
\bottomrule
\end{tabular}
\caption{Transferability of conditionally sampled weights across different ResNet architectures.}
\end{table}


==> tables/cross_dataset.tex <==
\begin{table}[t]
%\vskip -0.15in
\caption{\textbf{Cross-Dataset Trasfer} MNIST$\rightarrow$ SVHN, SVHN$\rightarrow$ MNIST, CIFAR-10$\rightarrow$ STL-10, STL-10 $\rightarrow$ CIFAR-10. The OFA model is pretrained on ImageNet.}
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{lcccc}
\toprule
Model & MNIST & SVHN & CIFAR10 & STL10 \\
\midrule
\midrule
Pretrained (seen) & 97.44& 84.04  &81.83  &66.62\\
D2NWG (seen) & 97.49& 83.12&82.19  &66.13\\ 
\midrule
OFA (Pretrained)\cite{cai2020once}& 13.34& 8.90&  13.34&  8.90\\
cross\_dataset (unseen) & \textbf{50.70} & 28.68  &34.16 & \textbf{39.95}\\
D2NWG (unseen) & 49.32& \textbf{29.13 } & \textbf{35.02 }
&39.90\\ 
D2NWG+average (unseen) & 50.24& \textbf{29.13 } & \textbf{35.03 }
&40.00\\ 
\bottomrule
\end{tabular}
}
\label{tabmbv3}
\vskip -0.15in
\end{table} 

==> tables/no_finet_tune_init.tex <==
% \begin{table}[t]
\begin{wraptable}{r}{8cm}
\vspace{-0.15in}
\caption{No Fine-tuning initialization on seen and unseen datasets. In the second row, baseline and pretrained weights we transfer the weights of MNIST model to SVHN and vice-versa similarly for STL-10 and CIFAR-10. For our method we use each of the datasets as unseen to generate the weights. }\label{crossall}
% \vspace{-0.25in}
\centering
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{lcccc}\\
\toprule  
Model & MNIST & SVHN & CIFAR10 & STL10 \\
\midrule
\midrule
RandInit &10.23 & 12.21 &9.98 & 9.56\\ 
Pretrained &  82.82 & \textbf{67.57}& \textbf{44.68} & \textbf{35.99}\\
S\textsubscript{\texttt{KDE30}} &  69.73& 50.25 & 26.06& 17.20\\
\midrule
Seen (D2NWG) &83.92 & 61.81 & 43.08& 31.45 \\ 
% Seen (D2NWG) (with Pred.) &84.85 & 66.03 & 43.89 & 34.29 \\ 
\midrule
S\textsubscript{\texttt{KDE30}} (Cross) &  29.30& 13.25 & 15.40& 15.20\\
% \midrule
Not seen (D2NWG) &36.64& 18.80& 18.00& 16.21\\ 
% Not seen (D2NWG) (with Pred.) &30.15 & 15.76& 17.10& 15.37\\ 
\bottomrule
\end{tabular}
}
\vspace{-0.2in}
% \end{table} 
\end{wraptable}

==> tables/unseen_real_world.tex <==
\begin{table*}%[t]
\vskip -0.10in
    \centering
    \caption{\textbf{Dataset Conditioned Sampling} Weight sampling on 10 unseen real-world datasets. We report two sets of results: (a) weight evaluation without finetuning and (b) weight evaluation after 50 epochs of finetuning. The pretrained baseline is trained on ImageNet1K. We report the accuracy on the testset.}
    \resizebox{0.8\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l|ccc|ccc}
    \toprule
       \multirow{2}{*}{Datasets} & \multicolumn{3}{c|}{Initialization} & \multicolumn{3}{c}{Fine-tuning} \\
        % \hline
         & RandInit& Pretrained & D2NWG & RandInit& Pretrained & D2NWG\\
        %\hline
        \midrule
        \midrule
        Gemstones & 1.13& 0.62  & \textbf{1.86 } & 70.59& 67.49 & \textbf{76.06 } \\
         %\hline
        Dog Breeds &0.55& 0.69  & \textbf{1.87} & 80.78& 78.13 & \textbf{80.88 } \\
         %\hline
        Dessert& 21.03 & 12.50  & \textbf{99.40 } & 95.83 & 94.64& \textbf{99.40}  \\
         %\hline
        Colorectal Histology& 11.77& 11.00 & \textbf{18.12 } & 90.34 & 89.75  & \textbf{93.65 }  \\
         %\hline
       Drawing&10.86  & 11.00  & \textbf{11.87 } & \textbf{90.20 }& 90.00 & 89.00 \\
        % \hline
        Alien vs Predator&51.48 & 28.88  & \textbf{78.15 } & 98.52& \textbf{98.89} & 97.77   \\
        % \hline
        COVID-19&20.13 & 46.53  & \textbf{47.22 } & 93.86& 93.40 & \textbf{94.56 } \\
        % \hline
        honey-bee-pollen&49.54& 50.00 &\textbf{56.94 } & 93.05 & 88.89 & \textbf{93.55  }  \\
        % \hline
        Speed Limit Signs& 30.55 & 25.00 &\textbf{31.48 } & 83.33& 86.11 & \textbf{90.74}  \\
        % \hline
        Japanese Characters&0.03 & 0.08 & \textbf{0.50} & 53.17 & \textbf{62.33} & 62.16 \\
         \bottomrule
    \end{tabular}
    }
    \label{tab2}
    \vskip -0.10in
\end{table*}

==> tables/zero_shot_mobilenet.tex <==
%\begin{wrapfigure}[11]{h}{0.6\textwidth}
%\small
%\centering
%\vspace{-0.15in}
%\captionof{table}{\small \textbf{Full-model weights generation} This Table represents results of zero-shot evaluation against the pretrained model on mobilenetv3 full model architecture weights sampling versus classifier layer weights sampling}
%\vspace{-0.1in}
%\resizebox{0.6\textwidth}{!}{
%\begin{tabular}{lcccc}
%\toprule
%Model & MNIST& SVHN & CIFAR-10 & STL-10\\
%\midrule
%Pretrained & 99.42 $\pm$ 0.05 & 94.62 $\pm$ 0.18 & 93.51 $\pm$ 0.16  &94.01 $\pm$ 0.10\\
%Linear\_prob & 96.88 $\pm$ 0.45 & 57.23 $\pm$ 0.28 & 82.85 $\pm$ 0.25  &95.63 $\pm$ 1.23\\
%\midrule
%D2NWG(prob) &  \textbf{99.55} $\pm$ \textbf{0.02} & \textbf{95.13} $\pm$ \textbf{0.10} & \textbf{94.23} $\pm$ \textbf{0.27} &94.02 $\pm$ 0.10\\
%D2NWG(full) &  97.56 $\pm$ 0.26 & 57.41 $\pm$ 0.17 & 83.64 $\pm$ 0.47  &\textbf{95.74} $\pm $ \textbf{0.74}\\
%\midrule
%Cross datasets transfer learning\\
%\midrule
%OFA (Pretrained)\cite{cai2020once}& 13.34& 8.90&  13.34&  8.90\\
%D2NWG(full) &  \textbf{66.82} $\pm$ \textbf{0.65} & \textbf{35.20} $\pm$ \textbf{0.65} & \textbf{36.70} $\pm$ \textbf{0.18}  & \textbf{51.50} $\pm$ \textbf{0.37}\\
%D2NWG(prob) &  42.86 $\pm$ 0.62 & 20.974 $\pm$ 0.78 & 26.56 $\pm$ 1.22  &47.33 $\pm$ 0.32\\
%\bottomrule
%\end{tabular}
%}
%\label{tab:mbv3}
%%\vspace{-0.1in}
%\end{wrapfigure}

\begin{table*}[t]
\caption{\small \textbf{Full-model weights generation} This Table represents results of zero-shot evaluation against the pretrained model on mobilenetv3 full model architecture weights sampling versus classifier layer weights sampling}
\vspace{-0.2in}
\begin{center}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{lcccc}
\toprule
Model & MNIST& SVHN & CIFAR-10 & STL-10\\
\midrule
Pretrained & 99.42 $\pm$ 0.05 & 94.62 $\pm$ 0.18 & 93.51 $\pm$ 0.16  &94.01 $\pm$ 0.10\\
Linear\_prob & 96.88 $\pm$ 0.45 & 57.23 $\pm$ 0.28 & 82.85 $\pm$ 0.25  &95.63 $\pm$ 1.23\\
\midrule
D2NWG(prob) &  \textbf{99.55} $\pm$ \textbf{0.02} & \textbf{95.13} $\pm$ \textbf{0.10} & \textbf{94.23} $\pm$ \textbf{0.27} &94.02 $\pm$ 0.10\\
D2NWG(full) &  97.56 $\pm$ 0.26 & 57.41 $\pm$ 0.17 & 83.64 $\pm$ 0.47  &\textbf{95.74} $\pm $ \textbf{0.74}\\
\midrule
Cross datasets transfer learning\\
\midrule
OFA (Pretrained)\cite{cai2020once}& 13.34& 8.90&  13.34&  8.90\\
D2NWG(full) &  \textbf{66.82} $\pm$ \textbf{0.65} & \textbf{35.20} $\pm$ \textbf{0.65} & \textbf{36.70} $\pm$ \textbf{0.18}  & \textbf{51.50} $\pm$ \textbf{0.37}\\
D2NWG(prob) &  42.86 $\pm$ 0.62 & 20.974 $\pm$ 0.78 & 26.56 $\pm$ 1.22  &47.33 $\pm$ 0.32\\
\bottomrule
\end{tabular}			
   }
\end{center}
\label{tab:mbv3}
\vspace{-0.2in}
\end{table*}

==> tables/zero_shot_vit_indist.tex <==

% \begin{wraptable}{r}{0.4\columnwidth}
\begin{table}[t]
% \vskip -0.15in
\caption{\textbf{Full vision transformer Paramters generation} This Table represent results of zero-shot evaluation against the pretrained model on VIT architecture}
\resizebox{0.4\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
Model & SVHN & CIFAR-10 & CIFAR-100 & CINI-10& Tiny-ImageNet \\
\midrule
\midrule
Pretrained (seen) & 97.73& 93.67  &83.56  &72.29& 53.36\\
D2NWG(ours) & \textbf{97.75 $\pm$ 0.01}& \textbf{93.70 $\pm$ 0.02} & \textbf{83.58 $\pm$ 00} & \textbf{72.75 $\pm$ 0.02} &\textbf{53.53 $\pm$ 0.05}\\ 
\bottomrule
\end{tabular}
}
\label{tabvit}
% \vskip -0.15in
\end{table} 
% \end{wraptable}
